Efficient and Eventually Consistent Collective Operations

Collective operations are common features of parallel programming models that are frequently used in High-Performance (HPC) and machine/ deep learning (ML/ DL) applications. In strong scaling scenarios, collective operations can negatively impact the overall application performance: with the increase in core count, the load per rank decreases, while the time spent in collective operations increases logarithmically. In this article, we propose a design for eventually consistent collectives suitable for ML/ DL computations by reducing communication in Broadcast and Reduce, as well as by exploring the Stale Synchronous Parallel (SSP) synchronization model for the Allreduce collective. Moreover, we also enrich the GASPI ecosystem with frequently used classic/ consistent collective operations -- such as Allreduce for large messages and AlltoAll used in an HPC code. Our implementations show promising preliminary results with significant improvements, especially for Allreduce and AlltoAll, compared to the vendor-provided MPI alternatives.

==> Collectives - arxiv-5/fig/conclusions.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}
In this article, we have adopted some classic algorithm for collective operations -- like Binomial Spanning Tree and segmented pipelined ring -- to implemented Broadcast, Reduce, and Allreduce with GASPI. While with Broadcast and Reduce we want to be generic, with Allreduce we are more specific and target (very) large message sizes. The Allreduce implementation leads to outstanding preliminary results compared to the vendor-specific implementation. We also implemented AlltoAll following a rather simple but well-performing pattern. Furthermore, we designed and implemented a novel Allreduce following the Stale Synchronous Parallel model, resulting in  {\tt allreduce\_ssp} thanks to GASPI. {\tt allreduce\_ssp} is suitable for ML/DL codes and is currently being tested with Bayesian Probabilistic Matrix Factorization. 
All our developments are available under the EPEEC GitHub repository: \url{https://github.com/epeec}.

Our ultimate goal is to provide a library of collectives within the GASPI ecosystem for both HPC and ML/DL communities by leveraging the GASPI API and focusing on the design of collectives for various data sizes and/or application needs as in case of the {\tt allreduce\_ssp} variant. Furthermore, we are also working on the compression library and foresee to design and develop another version of eventually consistent collectives by coupling this compression library and the classic collectives.  





==> fig/conclusions.tex <==
\section{Conclusions and Future Work}
\label{sec:conclusions}
In this article, we have adopted some classic algorithm for collective operations -- like Binomial Spanning Tree and segmented pipelined ring -- to implemented Broadcast, Reduce, and Allreduce with GASPI. While with Broadcast and Reduce we want to be generic, with Allreduce we are more specific and target (very) large message sizes. The Allreduce implementation leads to outstanding preliminary results compared to the vendor-specific implementation. We also implemented AlltoAll following a rather simple but well-performing pattern. Furthermore, we designed and implemented a novel Allreduce following the Stale Synchronous Parallel model, resulting in  {\tt allreduce\_ssp} thanks to GASPI. {\tt allreduce\_ssp} is suitable for ML/DL codes and is currently being tested with Bayesian Probabilistic Matrix Factorization. 
All our developments are available under the EPEEC GitHub repository: \url{https://github.com/epeec}.

Our ultimate goal is to provide a library of collectives within the GASPI ecosystem for both HPC and ML/DL communities by leveraging the GASPI API and focusing on the design of collectives for various data sizes and/or application needs as in case of the {\tt allreduce\_ssp} variant. Furthermore, we are also working on the compression library and foresee to design and develop another version of eventually consistent collectives by coupling this compression library and the classic collectives.  




